Stair Climbing using the Angular Momentum Linear Inverted Pendulum Model and Model Predictive Control

A new control paradigm using angular momentum and foot placement as state variables in the linear inverted pendulum model has expanded the realm of possibilities for the control of bipedal robots. This new paradigm, known as the ALIP model, has shown effectiveness in cases where a robot's center of mass height can be assumed to be constant or near constant as well as in cases where there are no non-kinematic restrictions on foot placement. Walking up and down stairs violates both of these assumptions, where center of mass height varies significantly within a step and the geometry of the stairs restrict the effectiveness of foot placement. In this paper, we explore a variation of the ALIP model that allows the length of the virtual pendulum formed by the robot's stance foot and center of mass to follow smooth trajectories during a step. We couple this model with a control strategy constructed from a novel combination of virtual constraint-based control and a model predictive control algorithm to stabilize a stair climbing gait that does not soley rely on foot placement. Simulations on a 20-degree of freedom model of the Cassie biped in the SimMechanics simulation environment show that the controller is able to achieve periodic gait.

==> Sections/Future.tex <==
\section{Future Work}
\label{sec:future}

This report shows there is much promise in the pendulum length-varying version of the ALIP model to handle terrain where the CoM height must vary. Here, we used ankle torque explicitly to stabilize Cassie's motion in the sagittal plane. Though not explored in this report, actively modifying the pendulum length may also be an effective control strategy. 

As discussed in Sec.~\ref{sec:mpc}, an important next step is to move from the na\"ive implementation of MPC used in this report to a more robust implementation of MPC that uses quadratic programming to solve for the optimization problem specifying the input torques. 

Additionally, implementing this control paradigm on the physical Cassie robot would also be in future work, as well as applying the controller on different bipedal systems such as RABBIT \cite{chevallereau2003rabbit} and Agility Robotics' Digit biped. This will prove the robustness of this control paradigm through its application on various systems. Furthermore, having the Cassie or Digit robots walk up the varying heights of stairs in the Robot Playground outside of the Ford Robotics Building would also further validate the robustness of the controllers.

Finally, collaborating with other members of the Biped Lab to incorporate computer vision to this work to make a bipedal robot move autonomously through loosely structured cluttered environments is another promising future direction.

==> Sections/archieve-Cassie.tex <==
\section{Controlling the Cassie Bipedal Robot}
\label{sec:control}

The Cassie robot (shown in Fig. \ref{fig:meandcassie}) is a 20 degree-of-freedom (DOF), 32 kg bipedal robot that was designed and built by the company Agility Robotics. Each of its 10 kg legs has 7 DOF, where 5 joints are actuated by motors and 2 are constrained by springs. Cassie's blade-shaped feet provide 5 holonomic constraints each when in contact with the ground.

\begin{figure}
    \centering
    \includegraphics[width=0.25\textwidth]{Media/MeandCassie2.PNG}
    \caption{Picture of the Cassie biped robot built by the company Agility Robotics as the author of this paper operates it.}
    \label{fig:meandcassie}
\end{figure}

%%%%%%      DYNAMICS      %%%%%%  
\subsection{Dynamics}
Bipedal locomotion, such as with stair climbing, can be best characterized using a \textit{hybrid system}--a system that displays both continuous and discrete behavior. The continuous phase describes the dynamics of one foot supporting the robot and the other swinging forward, while the discrete phase describes the transitions between left and right feet. The ``stance leg'' is defined as the leg that is planted on the ground during walking motion. Conversely, the ``swing leg'' refers to the leg whose foot is progressing forward.

Using Lagrangian mechanics, one obtains a second-order differential equation to describe the continuous dynamics for the Cassie biped:

\begin{equation}
D(q)\ddot{q} + C(q,\dot{q})\dot{q} + G(q) = J_{st}^TF + J_s^TF_s + Bu
\label{eq:eqofmotion}
\end{equation}
where $D \in \mathbb{R} ^{20 \times 20}$ is the mass inertial matrix, $C \in \mathbb{R}^{20 \times 20}$ is the centrifugal and coriolis forces matrix, $G \in \mathbb{R}^{20 \times 1}$ is the gravitational vector, $J_{st} \in \mathbb{R}^{5 \times 20}$ is the stance foot jacobian (I assume that the blade foot has two points of contact), $F \in \mathbb{R}^{5 \times 1}$ is the ground reaction force acting on the stance foot, $J_s \in \mathbb{R}^{4 \times 20}$ is the jacobian of the springs, $F_S \in \mathbb{R}^{4 \times 1}$ are the forces acting from the springs, $B \in \mathbb{R}^{20 \times 10}$ is the input matrix, $u \in \mathbb{R}^{10 \times 1}$ is the motor torque vector, and $q \in \mathbb{R}^{20 \times 1}$ is the generalized coordinate vector. 

%%%%%%      CONTROLLER      %%%%%%  
\subsection{Controller}
Input-Output Feedback Linearization is a common approach to control nonlinear systems such as bipedal robots \cite{westerveltfeedback}. Though the practical applications are limited due to computational constraints, its relatively simple nature makes it an ideal controller to use in simulation.

The output function is defined as
\begin{equation}
    y(x) = h(x) - h_d
    \label{eq:y}
\end{equation}
where $h$ is the virtual constraints and $h_d$ are the desired trajectories for the virtual constraints.

In part due to precedent \cite{gong2021,gibson2021,gong2019feedback} and in other part due to the new ALIP model that is being used for this paper, the virtual constraints are being defined as follows:

\begin{equation}
    h = 
    \begin{bmatrix}
    \text{absolute torso pitch}\\
    \text{absolute torso roll}\\
    \text{stance hip yaw}\\
    \text{swing hip yaw}\\
    \text{pendulum length}\\
    P_{st \to sw}^x\\
    P_{st \to sw}^y\\
    P_{st \to sw}^z\\
    \text{absolute swing toe pitch}
    \end{bmatrix}
    \label{eq:h}
\end{equation}
where the pendulum length describes the vector $r_c$ from the stance foot to the CoM and $P_{st \to sw}$ is the vector emanating from the stance and going to the swing foot.

I design a controller such that 

\begin{equation}
    \ddot{y} + K_D \dot{y} + K_P y = 0
    \label{eq:y_law}
\end{equation}
where $K_D$ and $K_P$ are user-defined derivative and proportional controller gains respectively.

The first and second derivatives of $y$ are defined as

\begin{equation}
    \begin{split}
        \dot{y} = -\dot{h}_d + Jh \dot{q}\\
        \ddot{y} = -\ddot{h}_d + Jh \ddot{q} + \delta Jh \dot{q}
    \end{split}
    \label{eq:hderivatives}
\end{equation}
where $Jh$ is the jacobian of the constraints $h$ at a given time step and $\delta J h$ is the partial derivative of the jacobian of the constraints at given time step with respect to $q$.

Plugging in Eq. \ref{eq:hderivatives} into Eq. \ref{eq:y_law} yields

\begin{equation}
    -\ddot{h}_d + Jh \ddot{q} + \delta J h \dot{q} + K_D(-\dot{h}_d + Jh \dot{q}) + K_P h = 0
    \label{eq:fullcontrollaw}
\end{equation}
where $\ddot{q}$ is known from the continuous dynamics defined in Eq. \ref{eq:eqofmotion}. That is,

\begin{equation}
    \begin{split}
        \ddot{q} = M([1:20],:)u - b[1:20]\\
        = \overline{M}u - \overline{b}
    \end{split}
    \label{eq:ddq}
\end{equation}
where $\overline{M}$ and $\overline{b}$ describe the first 20 rows of the matrices $M$ and $b$, which are defined as 
\begin{equation}
    \begin{split}
        M = 
        \begin{bmatrix}
            D & -J_{st}^T & -J_s^T \\
            J_{st} & 0 & 0 \\
            J_s & 0 & 0
        \end{bmatrix}^{-1}
        \begin{bmatrix}
            B\\
            0\\
            0
        \end{bmatrix}
        \\
        b = 
        \begin{bmatrix}
            D & -J_{st}^T & -J_s^T \\
            J_{st} & 0 & 0 \\
            J_s & 0 & 0
        \end{bmatrix}^{-1}
        \begin{bmatrix}
            C\dot{q}+G\\
            \dot{J}_{st}\dot{q}\\
            \dot{J}_s\dot{q}
        \end{bmatrix}.
    \end{split}
\end{equation}

Thus, plugging in Eq. \ref{eq:ddq} into Eq. \ref{eq:fullcontrollaw} and solving for the control input $u$, the final controller is defined as

\begin{equation}
    u = [Jh \overline{M}]^{-1} [\ddot{h}_d + Jh \overline{b} - \delta J h \dot{q} - K_D(-\dot{h}_d + J h\dot{q}) - K_P h].
\end{equation}

% %%%%%%      PENDULUM TRAJECTORY CONTROL      %%%%%%  
% \subsection{Pendulum Trajectory Control}
% The primary shortcoming of the old ALIP model is that it assumed constant CoM height, thereby making the model ineffective in situations where CoM height varies, such as with climbing stairs. While in previous work that has used the old ALIP model focused on attaining a desired angular momentum (and thus speed) at the end of a next step in a walking trajectory \cite{gong2021}\cite{gibson2021}\cite{gong2019feedback}, this work will seek to exploit the new ALIP model's main advantage over the old: independence from the robot's position with respect to its environment. The new model offers the opportunity to control a biped robot's gait using its CoM angle with respect to the stance foot, rather than foot placement, to control some desired variable at the end of the next step in a gait trajectory.

% To this end, I first used the Fast Robot Optimization and Simulation Toolkit (FROST) \cite{Hereid2017FROST} to generate a baseline optimized trajectory. I fitted a fourth order b\`ezier curve to the pendulum length trajectory $r_c$, as well as the other trajectories for the virtual constraints from Eq. \ref{eq:h}. Using just the optimized trajectory by itself proved to be ineffective to get the Cassie robot to walk up stairs in simulation. Among other problems, the controller could not maintain tracking with the optimized trajectory, in part due to Cassie losing momentum as it attempted to ascend the steps. This was caused by the vector from the stance foot to CoM getting longer over time, resulting in Cassie slowing down and eventually falling. Given the new formulation for the ALIP model as well as the nature of b\`ezier curves, an opportunity arose to modify the b\`ezier curve for the pendulum length in a manner such that the pendulum length would stay shorter toward the beginning and middle of a step, and increase in length at the end of the step to help generate the momentum needed to continue to the next step and beyond.

% In order to create this new ideal trajectory, I needed to modify the b\`ezier coefficients. At each time step of simulation, I selected the middle two b\`ezier coefficients from the original optimized trajectory from FROST. Using Euler integration and the new ALIP model defined in Eq. \ref{eq:newALIP}, I predicted the states $\theta_c$ and $L$ at the end of the current step if the two selected b\`ezier coefficients were increased or decreased by some small value $\delta$. Next, I applied an \textit{impact map} \cite{westerveltfeedback}, and then use Euler Integration and the new ALIP to find the states at the end of the next step in the trajectory. Recalling that the primary reason why momentum was being loss as Cassie ascended the stairs was due to the lengthening of the vector from the stance foot to the CoM $r_c$, I wanted to ensure that the angle of the CoM at the end of the next step was some desired value such that $r_c$ would not be too long. Using interpolation, I found the required $\delta$ value that I needed to change the two selected b\`ezier coefficients such that the desired CoM angle could be achieved by the end of the next step.

%%%%%%      Ankle Torque Control      %%%%%%  
\subsection{Stance Ankle Torque Control}
In previous work controlling the Cassie robot \cite{gong2021,gibson2021,gong2019feedback}, the stance ankle joint is typically left as passive by setting the stance ankle toque joint to zero. Climbing stairs requires substantial control effort that must go far beyond simply following an optimized trajectory, as will be addressed in Section \ref{sec:results}. To compensate for this deficiency, I strategically incorporated torque to the stance ankle motor to have the Cassie robot achieve and maintain a desired angular momentum and CoM angle. 

% Given angular momentum's relationship with velocity, this method also serves as a form of velocity control.

% To implement this additional control strategy, at each time step I first pick two torque values. Using Euler integration and the new ALIP model defined in Eq. \ref{eq:newALIP}, I predict the states $\theta_c$ and $L$ at the end of the current step. It should be noted that the derivative of angular momentum $\dot{L}$ about a contact point can be described as the summation of torques about that contact point. Thus, I add the new ankle torques to the dynamic model to account for the effects that it will have on the states of the robot. Next, I apply an impact map, and then use Euler Integration and the new ALIP to find the states at the end of the next step. In calculation to predict the states at the end of the next step, I do not include the new stance ankle torques since I only want to know the effects of the added torque if applied to the \textit{current} step.

% Using the values of the final angular momentum at the end of the next step for the two selected torques, I interpolate to find the desired ankle torque value that will achieve a desired angular momentum at the end of the next step.


% One reason for imposing these bounds is to prevent the desired torque value from spiking at the end of the current step. Recall that in the Euler Integration, the torque is only being applied to the current step to achieve a desired angular momentum at the end of the next step. If the model is unable to achieve a desired predicted angular momentum by the end of the current step, the controller would attempt to spike the ankle torques as the end of the current step approaches. Bounding torque will prevent this, giving the model permission to try to achieve the desired angular momentum by adding stance ankle torque in the next step.
To implement this control strategy in simulation, I needed to impose bounds on the stance ankle torque values. One reason for imposing bounds on the stance ankle torque values is to prevent rolling of the ankles. Consider the schematic of the Cassie robot's stance foot shown in Fig. \ref{fig:stanceFoot}. Note that I assume that the foot contacts the ground at two points. Given this set up, the total torque on the foot is

\begin{equation}
    \tau = F_2 L_2 - F_1 L_1.
    \label{eq:taustance}
\end{equation}

\begin{figure}
    \centering
    \includegraphics[width=0.25\textwidth]{Media/stanceFootTorque.png}
    \caption{Schematic of the forces and toque acting on the stance foot of Cassie.}
    \label{fig:stanceFoot}
\end{figure}

In order to increase the stance ankle torque $\tau$, $F_2$ must increase. Also note that since the only point of contact with the ground that the robot has is assumed to occur at these two points on the stance toe, $F_1$ and $F_2$ must add up to equal to the gravitational force on the robot. Thus,

\begin{equation}
    F_1 + F_2 = mg.
    \label{eq:stanceforce}
\end{equation}

Increasing $F_2$ means that $F_1$ must decrease in order for Eq. \ref{eq:stanceforce} to hold. $F_1$ cannot be negative (because the stance foot cannot be sucked into the ground), thus the minimum value that $F_1$ can be is zero. This implies that the maximum value that $F_2$ can be is $mg$.

Keep in mind that this is an extreme simplification of what an actual robot foot would look like, but it does provide useful insights for when determining the bounds for stance ankle torque input.

%%%%%%      FROST      %%%%%%  
\subsection{FROST}
The primary shortcoming of the old ALIP model is that it assumed constant CoM height, thereby making the model ineffective in situations where CoM height varies, such as with climbing stairs. While in previous work that has used the old ALIP model focused on attaining a desired angular momentum (and thus speed) at the end of a next step in a walking trajectory \cite{gong2021,powell2016,gibson2021,gong2019feedback}, this work seeks to exploit the new ALIP model's main advantage over the old: independence from the robot's position with respect to its environment. The new model offers the opportunity to control a biped robot's gait using its CoM angle with respect to the stance foot in addition to angular momentum about the contact point to control some desired variable (in this paper, stance ankle torque) throughout a gait trajectory.

To this end, I needed to use the Fast Robot Optimization and Simulation Toolkit (FROST) \cite{Hereid2017FROST} to generate a baseline optimized trajectory. I fitted a fourth order b\`ezier curve to the pendulum length trajectory $r_c$, as well as the other trajectories for the virtual constraints from Eq. \ref{eq:h}, CoM angle, and angular momentum about the contact point. 

Using just the optimized trajectory by itself proved to be ineffective to get the Cassie robot to walk up stairs in simulation. Among other problems, the controller can not maintain tracking with the optimized trajectory in part due to Cassie losing momentum as it ascends the steps. This was caused by the vector from the stance foot to CoM getting longer over time, resulting in Cassie slowing down and eventually falling. 

Setting desired states using the optimized trajectories generated with FROST, as well as adding stance ankle torque whose values are determined via MPC resolves this issue.

